Topmetal CMOS direct charge sensing plane for neutrinoless double-beta decay search in high-pressure gaseous TPC

We propose a novel charge sensing concept for high-pressure Time Projection Chamber (TPC) to search for Neutrinoless Double-Beta Decay (NLDBD) with ton-scale isotope mass and beyond. A meter-sized plane, tiled with an array of CMOS integrated sensors called Topmetal that directly collect charge without gas avalanche gain, is to be deployed into a high-pressure gaseous TPC with working gases containing suitable NLDBD candidate isotopes such as Xe-136 and Se-82. The Topmetal sensor has an electronic noise <30 e- per pixel, which allows the detector to reach <1% FWHM energy resolution at the NLDBD Q-value for both Xe-136 and 82SeF6 gases by measuring ionization charges alone. The elimination of charge avalanche gain allows the direct sensing of slow-drifting ions, which enables the use of highly electronegative gas SeF6 in which free electrons do not exist. It supports the swapping of working gases without hardware modification, which is a unique way to validate signals against radioactive backgrounds. Since the sensor manufacturing and plane assembling could leverage unaltered industrial mass-production processes, stability, uniformity, scalability, and cost-effectiveness that are required for ton-scale experiments could all be reached. The strengths of TPC such as 3D ionization tracking and decay daughter tagging are retained. This development could lead to a competitive NLDBD experiment at and above ton-scale. The conceptual considerations, simulations, and initial prototyping are discussed.

==> defs.tex <==
\usepackage{xspace}

% directory name
\newcommand{\dn}{.}

% font size
\makeatletter
% tex/latex/base/size10.clo
\newcommand\fontsizetenpt{%
   \@setfontsize\normalsize\@xpt\@xiipt
   \abovedisplayskip 10\p@ \@plus2\p@ \@minus5\p@
   \abovedisplayshortskip \z@ \@plus3\p@
   \belowdisplayshortskip 6\p@ \@plus3\p@ \@minus3\p@
   \belowdisplayskip \abovedisplayskip
   \let\@listi\@listI}
% tex/latex/base/size11.clo
\newcommand\fontsizeelevenpt{%
   \@setfontsize\normalsize\@xipt{13.6}%
   \abovedisplayskip 11\p@ \@plus3\p@ \@minus6\p@
   \abovedisplayshortskip \z@ \@plus3\p@
   \belowdisplayshortskip 6.5\p@ \@plus3.5\p@ \@minus3\p@
   \belowdisplayskip \abovedisplayskip
   \let\@listi\@listI}
\makeatother

% terms
\newcommand{\TE}{\ensuremath{t_\text{e}}\xspace}
\newcommand{\TF}{\ensuremath{t_\text{f}}\xspace}
\newcommand{\TM}{\emph{Topmetal}\xspace}
\newcommand{\TMI}{\mbox{\emph{Topmetal-I}}\xspace}
\newcommand{\TMII}{\mbox{\emph{Topmetal-II}}\xspace}
\newcommand{\TMIIm}{\mbox{\emph{Topmetal-II\raise0.5ex\hbox{-}}}\xspace}
\newcommand{\TMS}{\mbox{\emph{Topmetal-S}}\xspace}
\newcommand{\VR}{\ensuremath{V_\text{reset}}\xspace}
\newcommand{\ND}{``Node''\xspace}
\newcommand{\VN}{\ensuremath{V_\text{node}}\xspace}
\newcommand{\Vc}{\ensuremath{\Delta U}\xspace}
\newcommand{\benu}{\ensuremath{\beta\text{-}\nu}\xspace}
\newcommand{\abenu}{\ensuremath{a_{\beta\nu}}\xspace}
\newcommand{\HeSix}{\ensuremath{^6\text{He}}\xspace}
\newcommand{\dbd}{DBD\xspace}
\newcommand{\tnbb}{\ensuremath{2\nu\beta\beta}\xspace}
\newcommand{\znbb}{\ensuremath{0\nu\beta\beta}\xspace}
\newcommand{\Cf}{\ensuremath{C_f}\xspace}
\newcommand{\Cd}{\ensuremath{C_d}\xspace}
\newcommand{\MOLLER}{MOLLER\xspace}
\newcommand{\Moller}{M{\o}ller\xspace}
\newcommand{\PXIII}{\mbox{PandaX-III}\xspace}
\newcommand{\Amtfo}{\ce{^{241}Am}\xspace}
\newcommand{\Xeots}{\ce{^{136}Xe}\xspace}
\newcommand{\SeFs}{\ce{SeF6}\xspace}
\newcommand{\SeetFs}{\ce{^{82}SeF6}\xspace}
\newcommand{\Seet}{\ce{^{82}Se}\xspace}
\newcommand{\APV}{\ensuremath{A_{PV}}\xspace}
\newcommand{\Qbb}{\ensuremath{Q_{\beta\beta}}\xspace}
\newcommand{\RnD}{R\&D\xspace}
\newcommand{\mbb}{\ensuremath{m_{\beta\beta}}\xspace}

\DeclareSIUnit\keV{keV}
\DeclareSIQualifier\ee{ee}
\DeclareSIQualifier\nr{nr}
\DeclareSIUnit\pe{p.e.}

% for math
\newcommand{\vect}[1]{\mathbf{#1}}
\newtheorem{defn}{Definition}[section]
\newcommand{\GI}{G\!I}
%\newcommand{\Wr}{W\!r}
\newcommand{\Tw}{Tw}
\newcommand{\seq}[1]{{\tt #1}}
\DeclareMathOperator*{\erf}{erf}

% fixed-width table column
\usepackage{array}
\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{R}[1]{>{\raggedleft\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}

% misc command
\newcommand{\Mark}[1]{\textcolor{red}{#1}}
\newcommand{\repl}[2]{\textcolor{blue}{\textbf{#2}}\sout{\textcolor{gray}{#1}}}
\newcommand{\change}[1]{\textcolor{blue}{#1}}
\newcommand{\old}[1]{\textcolor{gray}{#1}}
\newcommand{\sym}[1]{\texttt{#1}}
% use the following as \begin{changemargin}{addtoleft}{addtoright} text \end{changemargin}
\def\changemargin#1#2{\list{}{\rightmargin#2\leftmargin#1}\item[]}
\let\endchangemargin=\endlist

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

